DiscoTK: Using Discourse Structure for Machine Translation Evaluation

We present novel automatic metrics for machine translation evaluation that use discourse structure and convolution kernels to compare the discourse tree of an automatic translation with that of the human reference. We experiment with five transformations and augmentations of a base discourse tree representation based on the rhetorical structure theory, and we combine the kernel scores for each of them into a single score. Finally, we add other metrics from the ASIYA MT evaluation toolkit, and we tune the weights of the combination on actual human judgments. Experiments on the WMT12 and WMT13 metrics shared task datasets show correlation with human judgments that outperforms what the best systems that participated in these years achieved, both at the segment and at the system level.

==> conclusions.tex <==
We have presented experiments in using discourse structure for improving
machine translation evaluation.  We first designed two
discourse-aware similarity measures, which used all-subtree
kernels to compare discourse parse trees in accordance with the
Rhetorical Structure Theory. Then, we have shown that these measures
can help improve a number of existing machine translation
evaluation metrics both at the segment- and the system-level.
Therefore, rather than proposing a single new metric, we have show that
discourse information is complementary to state-of-the-art evaluation 
metrics, and thus should be taken into account in the development of 
future richer evaluation measures.

Addressing discourse-level phenomena in MT is a relatively new research direction. Yet, many of the ongoing efforts have been moderately successful according to traditional evaluation metrics. There is a consensus in the MT community that more discourse-aware metrics need to be proposed for this area to move forward.
We believe this work to be a valuable contribution towards this goal.

%Here, we have presented experiments with a state-of-the-art RST discourse parser
%%which incorporates both the coherence structure and the lexical cohesion,
%and we define simple similarity measures based on all-subtree kernels,
%which can be used directly as evaluation metrics.
%Afterwards, we show how the discourse information embedded in both lexicalized and unlexicalized versions of these metrics can be valuable for MT evaluation.
%%

%In an extensive set of experiments on WMT12 and WMT11 data, we have observed that a variety of existing evaluation metrics, using various levels of linguistic information, can benefit from our discourse-aware metrics, both at the segment- and the system-level, especially when the discourse information is incorporated in an informed way (i.e., using tuning). Our results show that discourse parse trees can improve the state-of-the art MT metrics, and bring them closer to human perception of translation quality, even when we only use sentence-level discourse information.

The tuned combined metrics tested in this paper are just an initial proposal, consisting of simply adjusting the relative weights of the individual metrics in a linear combination. In the future, we plan to work on integrated representations of syntactic, semantic and discourse-based structures, which would allow us to train evaluation metrics based on more fine-grained features. Also in future work, we propose to use the discourse information for MT in two different ways.
First, at the sentence-level, we can use discourse information to rerank alternative MT hypotheses;
this could be applied either for MT parameter tuning, or as a post-processing step.
Second, we propose to move in the direction of using discourse information beyond the sentence level.


==> discussion.tex <==
- 6- Discussion\\
- - Depth of discourse analisys\\
- - - Does if fare better?\\
- - - Stress that more context is better\\



==> metrics.tex <==
Our working hypothesis is that the similarity between discourse structures provides information that can be valuable for evaluating MT systems. In particular, we believe that translations should preserve discourse relations. As an example, consider the three discourse trees (DTs) shown in Figure~\ref{fig:DTs}: (a) for a reference (human) translation, and (b) and (c) for translations of two different systems that participated in WMT12. Note that the \emph{Attribution} relation in the reference is also realized in the translation in (b), but not in (c), which makes (b) a better translation compared to (c),
according to our hypothesis. We argue that existing metrics that only use lexical and syntactic information cannot distinguish between the two correctly. %\red{(Am I making sense here?)}.

In order to develop a discourse-aware evaluation metric,
we first generate RST discourse trees for the reference and the system-translated sentences
using a discourse parser, and then we measure the similarity between the two discourse trees.
We describe these two steps below.

\begin{figure*}[bht]
  \centering
  \begin{subfigure}[t]{\textwidth}
  \centering
  \includegraphics[scale=0.7]{img/ref_51_b}
  \caption{A reference (human-generated) translation.}
  \end{subfigure}

 \begin{subfigure}[t]{\textwidth}
%  \begin{minipage}[b]{0.45\linewidth}
  \centering
  \includegraphics[scale=0.7]{img/qcri_51}
  \caption{A higher quality (system-generated) translation.}
  \end{subfigure}
%\end{minipage}

%\quad

  \begin{subfigure}[t]{\textwidth}
  \centering
  \includegraphics[scale=0.7]{img/kit_51}
  \caption{A lower quality (system-generated) translation.}
  \end{subfigure}
  \caption{Example of three different discourse trees for the translations of a source sentence. (a) The reference, (b) A higher quality translation, (c) A lower quality translation. [Source: WMT-2012]}
  \label{fig:DTs}
\end{figure*}


\subsection{Generating Discourse Trees} \label{sec: gen_dt}

In Rhetorical Structure Theory, discourse analysis involves two subtasks: \Ni {\it discourse segmentation}, or breaking the text into a sequence of clause-like units called elementary discourse units (EDUs), and \Nii{\it discourse parsing}, or the task of linking the units (EDUs and larger discourse units) into labeled discourse trees. Recently, \newcite{Shafiq12} proposed discriminative models for both discourse segmentation and discourse parsing at the sentence level. The segmenter uses a maximum entropy  model that achieves state-of-the-art accuracy on this task having an $F_1$-score of $90.5\%$ while human agreement is $98.3\%$.
     
The discourse parser uses a dynamic Conditional Random Field~\cite{Sutton07} as a \emph{parsing model} to infer the probability of all possible discourse tree constituents. The inferred (posterior) probabilities are then used in a probabilistic CKY-like bottom-up \emph{parsing algorithm} to find the most likely DT. Using the standard set of 18 coarse-grained relations defined in \cite{Carlson01}, the parser attains an $F_1$-score of 79.8\%, which is very close to the human agreement of 83\%. These high scores allowed us to develop successful discourse similarity metrics.    

%For \emph{discourse parsing}, they used
%%a probabilistic discriminative  with a large set of features, expressed as a
%s  The parsing model effectively represents the structure and the labels (i.e., relation) of a DT constituent jointly, and captures the sequential and hierarchical dependencies between them. 
%
%The parser is trained and tested on the standard RST-DT corpus \cite{Carlson02} containing 385 Wall Street Journal news articles (8272 sentences) taken fron the Penn Treebank corpus \cite{Marcus93}.  Since WMT evaluations were also performed on news domain, we expect similar performance when the discourse segmenter and the parser are applied to WMT datasets.

We experimented with two variations of the discourse trees --- \qcril  \ and \qcri. While in \qcril \ we include the lexical items (i.e., words), in \qcri \ we only consider the discourse relations. For example, the \qcri \ representation for the discourse tree in Figure \ref{fig:DTs}(a) is \emph{Elaboration$_{ROOT}$ (SPAN$_{Nuc}$)(Attribution$_{Sat}$ (SPAN$_{Sat}$)(SPAN$_{Nuc}$))}.

%\emph{Elaboration$_{ROOT}$ (SPAN$_{Nuc}$ (Voices)(are)(coming)(from)(Germany)(,))(Attribution$_{Sat}$ (SPAN$_{Sat}$ (suggesting))(SPAN$_{Nuc}$ (that)(ECB)(be)(the)(last)(resort)(creditor)(.)))}, and the \qcri \ representation for the same tree  is  \emph{Elaboration$_{ROOT}$ (SPAN$_{Nuc}$)(Attribution$_{Sat}$ (SPAN$_{Sat}$)(SPAN$_{Nuc}$))}.  
      

\subsection{Measuring Similarity}

A number of metrics have been proposed to measure the similarity between two labeled trees, e.g., Tree Edit Distance \cite{Tai79} and Tree Kernels \cite{Collins01,moschitti06}. Tree kernels (TKs) provide an effective way to integrate arbitrary tree structures in kernel-based machine learning algorithms like SVMs \cite{Vapnik95}. This allows to train evaluation metrics based on more fine-grained structural features.

%This allows us to compare two different trees (i.e. from an MT system and a reference). %tune the tree-based MT evaluation metrics from human judgments.

In our work, we use the convolution TK defined in \cite{Collins01}, which efficiently measures the number of common subtrees in two trees. Note that this kernel was originally designed for syntactic parsing, and the subtrees are subject to the constraint that their nodes are taken with all or none of the children. To suit the kernel well to the discourse trees, we made a simple modification. More specifically, when we compare two subtrees, we disregard the nuclearity statuses of their respective roots since they do not contribute to the subtrees under consideration. For instance, this modification allows the kernel to find the subtree \emph{Attribution (SPAN$_{Sat}$, SPAN$_{Nuc}$)} common in (a) and (b) in Figure \ref{fig:DTs}.

 





==> related.tex <==

Addressing discourse-level phenomena in MT is relatively new as a research direction.
%Previously, discourse-related concepts such as lexical choice \cite{Carpuat2009,Voigt2012},
%and WSD \cite{Carpuat2007} have been addressed in MT.
%In recent years,
Some recent work has looked at anaphora resolution \cite{Hardmeier2010}
and discourse connectives~\cite{Cartoni2011,Meyer2011},
to mention two examples.\footnote{We refer the reader to~\cite{Hardmeier2012}
for an in-depth overview of discourse-related research for MT.}
However, so far the attempts to incorporate discourse-related knowledge in MT
have been only moderately successful, at best.
A common argument, is that current automatic evaluation metrics such as \bleu \ 
are inadequate to capture discourse-related aspects of translation quality~\cite{Meyer2012,Hardmeier2010}.
Thus, there is a consensus that discourse-informed MT evaluation metrics are needed
in order to advance research in this direction.
Here we suggest some simple ways to create such metrics and
we also show that they yield better correlation with human judgments.
%Indeed, in this work, we show that additional linguistic knowledge related to discourse
%structures can improve existing MT evaluation metrics.

The field of automatic evaluation metrics for MT is very active, and new metrics are
continuously being proposed, especially in the context of evaluation campaigns
run as part of the 
%the \emph{evaluation tasks} from the series of
Workshops on Statistical Machine Translation (WMT 2008-2012),
the NIST Metrics for Machine Translation Challenge (MetricsMATR), etc.
For example, at WMT12, 12 metrics were compared \cite{WMT12}, most of them new.

There have been several attempts to incorporate 
syntactic and semantic linguistic knowledge into MT evaluation.
For example, in the syntactic case, we find metrics that measure the structural similarity between
shallow syntactic sequences \cite{Gimenez2007,Popovic2007} or between constituency trees \cite{Liu2005}.
In the semantic case, there are metrics that exploit the similarity over named entities
and predicate-argument structures~\cite{Gimenez2007,Lo2012},

% or semantic frames~\cite{Lo2011}.
% Lluís1: sematic frames = SRL = predicate argument structure
% Lluís2: Lo2011 introduced MEANT which is semi-automatic; the fully automatic metric is "UMEANT" from 2012
% Reference to be added (@Paco, Lo2012):
%   Chi-kiu Lo and Dekai Wu. Unsupervised vs.
%   supervised weight estimation for semantic MT
%   evaluation metrics. In Proceedings of the 6th
%   Workshop on Syntax and Structure in Statistical
%   Translation (SSST-6), 2012.
% Lluís3: If we need space we can substitute "Gimenez2007" by "AsiyaMTjournal", which also describes and uses
% these metrics and it is already in the bibliography.
%

%\alert{There are many more linguistically-rich metrics (e.g., based on textual entailment features;
%those from Singapore, etc.), but I guess that with the current sample is enough.}

In the present work, instead of proposing a new metric, we focus on enriching current 
MT evaluation metrics with discourse information. We observe that many existing metrics
can benefit from additional knowledge about discourse structure.

In comparison to the syntactic and semantic extensions of MT metrics,
there have been very few efforts to incorporate discourse information so far.
%  had only been evaluated in small datasets.
One example are the semantics-aware metrics of \newcite{Gimenez2009} and \newcite{Comelles2010},
which use the Discourse Representation Theory~\cite{Kamp1993}
and tree-based discourse representation structures (DRS) produced by a semantic parser.
They calculate the similarity between the MT output and references
based on DRS subtree matching, as defined in~\cite{Liu2005},
DRS lexical overlap,
and DRS morpho-syntactic overlap.
However, they could not improve correlation with human judgments,
as evaluated on the MetricsMATR dataset (consisting of 249 manually-assessed segments).
%The evaluation on the MetricsMATR dataset\footnote{It consists of 249 manually assessed segments:
%at the system- and the document-level.}
%(document-level human assessments were produced by aggregating over segment-level judgments).
%They observed that the metric using DRS structures did not achieve any improvement in both settings in
%terms of the correlation with human judgments.

Compared to their work,
\Ni \ we use a different discourse representation (RST),
\Nii \ we compare discourse parses using \emph{all-subtree} kernels \cite{Collins01},
\Niii \ we evaluate on much larger datasets, for several language pairs and for multiple metrics,
and
\Niv \ we do demonstrate better correlation with human judgments.
%\Niv our discourse analysis is still circumscribed to the sentence level.

\newcite{Wong2012} recently proposed an extension of MT metrics
%such as \bleu, \ter \ and \meteor \
with a measure of document-level \emph{lexical cohesion} \cite{Halliday76}.
Lexical cohesion is achieved using word repetitions
and semantically similar words such as synonyms, hypernyms, and hyponyms.
For \bleu \ and \ter, they observed improved correlation with human judgments on the MTC4 dataset (900 segments)
when linearly interpolating these metrics with their \emph{lexical cohesion} score.
%However, they ignore the key property of a discourse, i.e., \emph{the coherence structure}, which we effectively exploit in both tuning and no-tuning scenarios. Furthermore, we show that the similarity in discourse trees can yield improvements in a larger number of existing MT evaluation metrics.
Unlike in Wong and Kit's work, which measures lexical cohesion at the document-level,
here we are concerned with \emph{coherence (rhetorical) structure},
primarily at the sentence-level.


%Two complementary aspects of discourse work together to make it interpretable as a whole. Similarly, in this work, we showcase the improvements in correlation both at a system and segment level when using discourse similarity as an additional metric component. However, in the present paper, we show results that use discourse structure at a sentence-level, and that improve the correlation in most of the metrics of the WMT-12 metrics evaluation shared task, at a segment and system level.

%\alert{This last part of the paragraph is not very convincing to me. Shouldn't we say that the main
%conceptual difference is that they are trying to measure cohesion at document level and we are more concerned
%with discourse (rhetorical) structure? Shafiq?}




==> results.tex <==
%----------------------------------------
% Discourse Parsing for MT Evaluation
% Subsection: Results
% Guzmán - Joty - Marquez - Nakov, January 2014
%----------------------------------------

%\textbf{Preslav: I have several comments in the LaTeX itself, marked with "Preslav:". Have a look!}

Below we present the evaluation results at the system- and segment-level.
We try both simple linear and tuned combinations.
Moreover, we experiment with tuning on WMT12 and testing on WMT11. 
Our two basic metrics on discourse trees (Section \ref{sec: gen_dt}) are 
referred to as \qcril\ and \qcri.

\begin{table*}[t]
\begin{center}
{\small\begin{tabular}{@{}r|r@{ }@{ }r@{ }@{ }r|r@{ }@{ }r@{ }@{ }r|r@{ }@{ }r@{ }@{ }r|r@{ }@{ }r@{ }@{ }r|r@{ }@{ }r@{ }@{ }r|@{}}
\cline{2-16}
& \multicolumn{3}{c}{\csen} & \multicolumn{3}{|c}{\deen} & \multicolumn{3}{|c}{\esen} & \multicolumn{3}{|c}{\fren} & \multicolumn{3}{|c|}{Average}\\
\cline{2-16}
Metrics &  & +\sqcri & +\sqcril &  & +\sqcri & +\sqcril &  & +\sqcri & +\sqcril &  & +\sqcri & +\sqcril &  & +\sqcri & +\sqcril\\
\hline
\qcri & .257 & -- & -- & .647 & -- & -- & .825 & -- & -- & .639 & -- & -- & .592 & -- & -- \\
\qcril & .371 & -- & -- & .682 & -- & -- & .972 & -- & -- & .800 & -- & -- & .706 & -- & -- \\
\hline
%0.902   SEMPOS                  0.943   0.924   0.937   0.804
%0.897   DR-QCRI-0:SEMPOS_norm   0.886   0.924   0.937   0.843
%0.826   DR-QCRI-2:SEMPOS_norm   0.714   0.874   0.923   0.793
\sempos & .943 & \emph{.886} & \emph{.714} & .924 & .924 & \emph{.874} & .937 & .937 & \emph{.923} & .804 & \bf .843 & \emph{.793} & .902 & \emph{.897} & \emph{.826} \\
%0.857   AMBER                   0.829   0.785   0.965   0.85
%0.869   DR-QCRI-0:AMBER_norm    0.829   0.835   0.979   0.832
%0.775   DR-QCRI-2:AMBER_norm    0.657   0.75    0.916   0.779
\amber & .829 & .829 & \emph{.657} & .785 & \bf .835 & \emph{.750} & .965 & \bf .979 & \emph{.916} & .850 & \emph{.832} & \emph{.779} & .857 & \bf .869 & \emph{.775} \\
%0.834   Meteor                  0.657   0.885   0.951   0.843
%0.840   DR-QCRI-0:Meteor_norm   0.6     0.912   0.986   0.861
%0.760   DR-QCRI-2:Meteor_norm   0.6     0.762   0.916   0.761
\meteor & .657 & \emph{.600} & \emph{.600} & .885 & \bf .912 & \emph{.762} & .951 & \bf .986 & \emph{.916} & .843 & \bf .861 & \emph{.761} & .834 & \bf .840 & \emph{.760} \\
%0.831   TerrorCat                        0.714   0.762   0.965   0.882
%0.786   DR-QCRI-0:TerrorCat_norm        -0.886  -0.476  -0.951  -0.832
%0.538   DR-QCRI-2:TerrorCat_sum         -0.657  -0.126  -0.580  -0.789
\terrorcat & .714 & \bf -.886 & \emph{-.657} & .762 & \emph{-.476} & \emph{-.126} & .965 & \emph{-.951} & \emph{-.580} & .882 & \bf -.832 & \emph{-.789} & .831 & \emph{.786} & \emph{.538} \\
%0.823   SIMPBLEU                        0.886   0.697   0.888   0.821
%0.832   DR-QCRI-0:SIMPBLEU_norm         0.829   0.765   0.902   0.832
%0.741   DR-QCRI-2:SIMPBLEU_norm         0.657   0.621   0.881   0.807
\simpbleu & .886 & \emph{.829} & \emph{.657} & .697 & \bf .765 & \emph{.621} & .888 & \bf .902 & \emph{.881} & .821 & \bf .832 & \emph{.807} & .823 & \bf .832 & \emph{.741} \\
%0.812   TER                    -0.886  -0.624  -0.916  -0.821
%0.844   DR-QCRI-0:TER_norm      0.886   0.709   0.951   0.829
%0.795   DR-QCRI-2:TER_norm      0.829   0.609   0.923   0.818
\ter & -.886 & .886 & \emph{.829} & -.624 & \bf .709 & \emph{.609} & -.916 & \bf .951 & \bf .923 & -.821 & \bf .829 & \emph{.818} & .812 & \bf .844 & \emph{.795} \\
%0.810   BLEU_4_closest_cased                    0.886   0.671   0.874   0.811
%0.822   DR-QCRI-0:BLEU_4_closest_cased_norm     0.886   0.679   0.895   0.829
%0.783   DR-QCRI-2:BLEU_4_closest_cased_norm     0.829   0.618   0.881   0.804
\bleu & .886 & .886 & \emph{.829} & .671 & \bf .679 & \emph{.618} & .874 & \bf .895 & \bf .881 & .811 & \bf .829 & \emph{.804} & .810 & \bf .822 & \emph{.783} \\
%0.754   posF                    0.657   0.662   0.874   0.825
%0.767   DR-QCRI-0:posF_norm     0.543   0.774   0.881   0.871
%0.696   DR-QCRI-2:posF_sum      0.543   0.624   0.846   0.771
\posf & .657 & \emph{.543} & \emph{.543} & .662 & \bf .774 & \emph{.624} & .874 & \bf .881 & \emph{.846} & .825 & \bf .871 & \emph{.771} & .754 & \bf .767 & \emph{.696} \\
%0.751   BlockErrCats                   -0.638  -0.747  -0.881  -0.738
%0.749   DR-QCRI-0:BlockErrCats_norm     0.6     0.771   0.881   0.746
%0.740   DR-QCRI-2:BlockErrCats_norm     0.6     0.741   0.874   0.746
\block & -.638 & \emph{.600} & \emph{.600} & -.747 & \bf .771 & \emph{.741} & -.881 & .881 & \emph{.874} & -.738 & \bf .746 & \bf .746 & .751 & \emph{.749} & \emph{.740} \\
%0.738   WordBlockErrCats                       -0.657  -0.674  -0.853  -0.768
%0.752   DR-QCRI-0:WordBlockErrCats_norm         0.657   0.709   0.853   0.789
%0.709   DR-QCRI-2:WordBlockErrCats_norm         0.6     0.685   0.846   0.704
\word & -.657 & .657 & \emph{.600} & -.674 & \bf .709 & \bf .685 & -.853 & .853 & \emph{.846} & -.768 & \bf .789 & \emph{.704}  & .738 & \bf .752 & \emph{.709} \\
%0.735   XEnErrCats                     -0.657  -0.638  -0.874  -0.771
%0.743   DR-QCRI-0:XEnErrCats_norm       0.657   0.662   0.874   0.779
%0.725   DR-QCRI-2:XEnErrCats_norm       0.657   0.618   0.846   0.779
\xen & -.657 & .657 & .657 & -.638 & \bf .662 & \emph{.618} & -.874 & .874 & \emph{.846} & -.771 & \bf .779 & \bf .779 & .735 & \bf .743 & \emph{.725} \\
\hline
%0.817   NIST            0.943   0.682   0.832   0.811
%0.864   DR-QCRI-0:NIST  0.886   0.75    0.979   0.839
%0.763   DR-QCRI-2:NIST  0.657   0.644   0.923   0.829
\nist & .943 & \emph{.886} & \emph{.657} & .682 & \bf .750 & \emph{.644} & .832 & \bf .979 & \bf .923 & .811 & \bf .839 & \bf .829 & .817 & \bf .864 & \emph{.763} \\
%0.884   ROUGE-W                 1.0     0.765   0.965   0.807
%0.887   DR-QCRI-0:ROUGE-W       0.886   0.859   0.965   0.839
%0.767   DR-QCRI-2:ROUGE-W       0.6     0.756   0.923   0.789
\rouge & 1.00 & \emph{.886} & \emph{.600} & .765 & \bf .859 & \emph{.756} & .965 & .965 & \emph{.923} & .807 & \bf .839 & \emph{.789} & .884 & \bf .887 & \emph{.767} \\
\hline
%0.876   LEXICAL                 0.943   0.776   0.944   0.843
%0.876   DR-QCRI-0:LEXICAL       0.943   0.776   0.944   0.843
%0.870   DR-QCRI-2:LEXICAL       0.943   0.768   0.93    0.839
\lex & .943 & .943 & .943 & .776 & .776 & \emph{.768} & .944 & .944 & \emph{.930} & .843 & .843 & \emph{.839} & .876 & .876 & \emph{.870} \\
%0.893   PARSING                 0.943   0.903   0.902   0.825
%0.899   DR-QCRI-0:PARSING       0.943   0.918   0.902   0.832
%0.878   DR-QCRI-2:PARSING       0.886   0.894   0.902   0.829
\syn & .943 & .943 & \emph{.886} & .903 & \bf .918 & \emph{.894} & .902 & .902 & .902 & .825 & \bf .832 & \bf .829 & .893 & \bf .899 & \emph{.878} \\
%0.910   SEMANTIC_ROLES                  0.943   0.888   0.965   0.843
%0.913   DR-QCRI-0:SEMANTIC_ROLES        0.943   0.9     0.965   0.843
%0.906   DR-QCRI-2:SEMANTIC_ROLES        0.943   0.891   0.965   0.825
\srl & .943 & .943 & .943 & .888 & \bf .900 & \bf .891 & .965 & .965 & .965 & .843 & .843 & \emph{.825} & .910 & \bf .913 & \emph{.906} \\
%0.893   DISCOURSE               0.886   0.894   0.93    0.861
%0.896   DR-QCRI-0:DISCOURSE     0.886   0.897   0.93    0.871
%0.838   DR-QCRI-2:DISCOURSE     0.714   0.865   0.93    0.843
\dis & .886 & .886 & \emph{.714} & .894 & \bf .897 & \emph{.865} & .930 & .930 & .930 & .861 & \bf .871 &\emph{.843} & .893 & \bf .896 & \emph{.838} \\
%0.905   ULC2                    0.943   0.891   0.951   0.836
%0.909   DR-QCRI-0:ULC2          0.943   0.906   0.951   0.836
%0.909   ALL2009-DR-QCRI-2       0.943   0.891   0.951   0.85
\asiyaix & .943 & .943 & .943 & .891 & \bf .906 & .891 & .951 & .951 & .951 & .836 & .836 & \bf .850 & .905 & \bf .909 & \bf .909 \\
%0.886   ULC             0.943   0.821   0.944   0.836
%0.900   DR-QCRI-0:ULC   0.943   0.879   0.944   0.836
%0.891   ALL-DR-QCRI-2   0.943   0.826   0.944   0.85
\asiyaall & .943 & .943 & .943 & .821 & \bf .879 & \bf .826 & .944 & .944 & .944 & .836 & .836 & \bf .850 & .886 & \bf .900 & \bf .891 \\
\hline
AVERAGE & .840 & .823 & .735 & .773 & .795 & .714 & .916 & .930 & .889 & .821 & .831 & .800 & .837 & .844 & .785\\
diff &  & -.017 & -.104 &  & +.022 & -.059 &  & +.014 & -.027 &  & +.010 & -.021 &  & +.007 & -.053\\
\hline
\end{tabular}}
\end{center}
\caption{\label{tab:results-wmt12-sys}Results on WMT12 at the system level. Pearson correlation with human judgments.}
\end{table*}


\begin{table*}[t]
\begin{center}
{\small\begin{tabular}{@{}r|r@{ }@{ }r@{ }@{ }r|r@{ }@{ }r@{ }@{ }r|r@{ }@{ }r@{ }@{ }r|r@{ }@{ }r@{ }@{ }r|r@{ }@{ }r@{ }@{ }r|@{}}
\cline{2-16}
& \multicolumn{3}{c}{\csen} & \multicolumn{3}{|c}{\deen} & \multicolumn{3}{|c}{\esen} & \multicolumn{3}{|c}{\fren} & \multicolumn{3}{|c|}{Average}\\
\cline{2-16}
Metrics &  & +\sqcri & +\sqcril &  & +\sqcri & +\sqcril &  & +\sqcri & +\sqcril &  & +\sqcri & +\sqcril &  & +\sqcri & +\sqcril\\
\hline
%-0.422  DR-QCRI-0       -0.473(11594)   -0.369(11934)   -0.436(9796)    -0.410(11021)
\qcri & -.473 & -- & -- & -.369 & -- & -- & -.436 & -- & -- & -.410 & -- & -- & -.422 & -- & -- \\
%0.165   DR-QCRI-2       0.173(11594)    0.162(11934)    0.180(9796)     0.145(11021)
\qcril & .173 & -- & -- & .162 & -- & -- & .180 & -- & -- & .145 & -- & -- & .165 & -- & -- \\
\hline
%0.254   spede07_pP                      0.260(11594)    0.278(11934)    0.265(9796)     0.212(11021)
%0.174   DR-QCRI-0:spede07_pP_norm       0.185(11594)    0.186(11934)    0.195(9796)     0.132(11021)
%0.225   DR-QCRI-2:spede07_pP_norm       0.232(11594)    0.229(11934)    0.246(9796)     0.192(11021)
\spede & .260 & \emph{.185} & \emph{.232} & .278 & \emph{.186} & \emph{.229} & .265 & \emph{.195} & \emph{.246} & .212 & \emph{.132} & \emph{.192} & .254 & \emph{.174} & \emph{.225} \\
%0.247   Meteor                  0.251(11594)    0.275(11934)    0.249(9796)     0.212(11021)
%0.173   DR-QCRI-0:Meteor_norm   0.183(11594)    0.186(11934)    0.185(9796)     0.140(11021)
%0.232   DR-QCRI-2:Meteor_norm   0.241(11594)    0.243(11934)    0.243(9796)     0.202(11021)
\meteor & .251 & \emph{.183} & \emph{.241} & .275 & \emph{.186} & \emph{.243} & .249 & \emph{.185} & \emph{.243} & .212 & \emph{.140} & \emph{.202} & .247 & .\emph{173} & \emph{.232} \\
%0.229   AMBER                   0.245(11594)    0.248(11934)    0.231(9796)     0.191(11021)
%0.178   DR-QCRI-0:AMBER_norm    0.201(11594)    0.189(11934)    0.186(9796)     0.137(11021)
%0.224   DR-QCRI-2:AMBER_norm    0.238(11594)    0.233(11934)    0.231(9796)     0.195(11021)
\amber & .245 & \emph{.201} & \emph{.238} & .248 & \emph{.189} & \emph{.233} & .231 & \emph{.186} & .231 & .191 & \emph{.137} & \bf .195 & .229 & \emph{.178} & \emph{.224} \\
%0.172   SIMPBLEU                0.193(11594)    0.172(11934)    0.189(9796)     0.134(11021)
%0.133   DR-QCRI-0:SIMPBLEU_norm 0.153(11594)    0.142(11934)    0.149(9796)     0.088(11021)
%0.208   DR-QCRI-2:SIMPBLEU_norm 0.226(11594)    0.206(11934)    0.223(9796)     0.177(11021)
\simpbleu & .193 & \emph{.153} & \bf .226 & .172 & \emph{.142} & \bf .206 & .189 & \emph{.149} & \bf .223 & .134 & \emph{.088} & \bf .177 & .172 & \emph{.133} & \bf .208 \\
%0.165   XEnErrCats                      0.174(11594)    0.184(11934)    0.177(9796)     0.127(11021)
%0.127   DR-QCRI-0:XEnErrCat_norm        0.141(11594)    0.139(11934)    0.141(9796)     0.087(11021)
%0.196   DR-QCRI-2:XEnErrCat_norm        0.210(11594)    0.191(11934)    0.208(9796)     0.174(11021)
\xen & .174 & \emph{.141} & \bf .210 & .184 & \emph{.139} & \bf .191 & .177 & \emph{.141} & \bf .208 & .127 & \emph{.087} & \bf .174 & .165 & \emph{.127} & \bf .196 \\
%0.154   posF                    0.158(11594)    0.185(11934)    0.152(9796)     0.122(11021)
%0.122   DR-QCRI-0:posF_norm     0.123(11594)    0.142(11934)    0.140(9796)     0.084(11021)
%0.210   DR-QCRI-2:posF_norm     0.223(11594)    0.223(11934)    0.219(9796)     0.173(11021)
\posf & .158 & \emph{.123} & \bf .223 & .185 & \emph{.142} & \bf .223 & .152 & \emph{.140} & \bf .219 & .122 & \emph{.084} & \bf .173 & .154 & \emph{.122} & \bf .210 \\
%0.153   WordBlockErrCats                0.152(11594)    0.161(11934)    0.168(9796)     0.130(11021)
%0.118   DR-QCRI-0:WordBlockErrCats_norm 0.126(11594)    0.119(11934)    0.134(9796)     0.092(11021)
%0.199   DR-QCRI-2:WordBlockErrCats_norm 0.206(11594)    0.203(11934)    0.218(9796)     0.168(11021)
\word & .152 & \emph{.126} & \bf .206 & .161 & \emph{.119} & \bf .203 & .168 & \emph{.134} & \bf .218 & .130 & \emph{.092} & \bf .168 & .153 & \emph{.118} & \bf .199 \\
%0.074   BlockErrCats                    0.068(11594)    0.082(11934)    0.084(9796)     0.063(11021)
%0.062   DR-QCRI-0:BlockErrCats_norm     0.057(11594)    0.072(11934)    0.073(9796)     0.046(11021)
%0.173   DR-QCRI-2:BlockErrCats_norm     0.177(11594)    0.172(11934)    0.191(9796)     0.153(11021)
\block & .068 & \emph{.057} & \bf .177 & .082 & \emph{.072} & \bf .172 & .084 & \emph{.073} & \bf .191 & .063 & \emph{.046} & \bf .153 & .074 & \emph{.062} & \bf .173 \\
%-0.186  TerrorCat                       -0.178(11594)   -0.195(11934)   -0.184(9796)    -0.186(11021)
%-0.115  DR-QCRI-0:TerrorCat_norm        -0.108(11594)   -0.099(11934)   -0.111(9796)    -0.141(11021)
%-0.084  DR-QCRI-2:TerrorCat_norm        -0.041(11594)   -0.096(11934)   -0.088(9796)    -0.112(11021)
\terrorcat & -.178 & \bf -.108 & \bf -.041 & -.195 & \bf -.099 & \bf -.096 & -.184 & \bf -.111 & \bf -.088 & -.186 & \bf -.141 & \bf -.112 & -.186 & \bf -.115 & \bf -.084 \\
\hline
%0.214   NIST            0.222(11594)    0.232(11934)    0.205(9796)     0.197(11021)
%0.168   DR-QCRI-0:NIST  0.184(11594)    0.182(11934)    0.166(9796)     0.141(11021)
%0.214   DR-QCRI-2:NIST  0.228(11594)    0.220(11934)    0.219(9796)     0.189(11021)
\nist & .222 & \emph{.184} & \bf .228 & .232 & \emph{.182} & \emph{.220} & .205 & \emph{.166} & \bf .219 & .197 & \emph{.141} & \emph{.189} & .214 & \emph{.168} & .214 \\
%0.185   ROUGE-W                 0.205(11594)    0.186(11934)    0.197(9796)     0.151(11021)
%0.136   DR-QCRI-0:ROUGE-W       0.156(11594)    0.138(11934)    0.154(9796)     0.097(11021)
%0.211   DR-QCRI-2:ROUGE-W       0.230(11594)    0.207(11934)    0.228(9796)     0.180(11021)
\rouge & .205 & \emph{.156} & .230 & .186 & \emph{.138} & \bf .207 & .197 & \emph{.154} & \bf .228 & .151 & \emph{.097} & \bf .180 & .185 & \emph{.136} & \bf .211 \\
%0.218   TERp-A                  0.209(11594)    0.254(11934)    0.229(9796)     0.178(11021)
%0.177   DR-QCRI-0:TERp-A        0.185(11594)    0.202(11934)    0.185(9796)     0.135(11021)
%0.244   DR-QCRI-2:TERp-A        0.240(11594)    0.264(11934)    0.269(9796)     0.204(11021)
\ter & .209 & \emph{.185} & \bf .240 & .254 & \emph{.202} & \bf .264 & .229 & \emph{.185} & \bf .269 & .178 & \emph{.135} & \bf .204 & .218 & \emph{.177} & \bf .244 \\
%0.185   BLEU            0.209(11594)    0.186(11934)    0.186(9796)     0.159(11021)
%0.149   DR-QCRI-0:BLEU  0.172(11594)    0.152(11934)    0.160(9796)     0.111(11021)
%0.206   DR-QCRI-2:BLEU  0.232(11594)    0.198(11934)    0.216(9796)     0.178(11021)
\bleu & .209 & \emph{.172} & \bf .232 & .186 & \emph{.152} & \bf .198 & .186 & \emph{.160} & \bf .216 & .159 & \emph{.111} & \bf .178 & .185 & \emph{.149} & \bf .206 \\
\hline
%0.254   LEXICAL                 0.258(11594)    0.277(11934)    0.258(9796)     0.224(11021)
%0.235   DR-QCRI-0:LEXICAL       0.244(11594)    0.252(11934)    0.244(9796)     0.201(11021)
%0.257   DR-QCRI-2:LEXICAL       0.264(11594)    0.272(11934)    0.267(9796)     0.225(11021)
\lex & .258 & \emph{.244} & \bf .264 & .277 & \emph{.252} & \emph{.272} & .258 & \emph{.244} & \bf .267 & .224 & \emph{.201} & \bf .225 & .254 & \emph{.235} & \bf .257 \\
%0.177   PARSING                 0.186(11594)    0.189(11934)    0.186(9796)     0.149(11021)
%0.167   DR-QCRI-0:PARSING       0.177(11594)    0.179(11934)    0.183(9796)     0.129(11021)
%0.198   DR-QCRI-2:PARSING       0.206(11594)    0.207(11934)    0.211(9796)     0.169(11021)
\syn & .186 & \emph{.177} & \bf .206 & .189 & \emph{.179} & \bf .207 & .186 & \emph{.183} & \bf .211 & .149 & \emph{.129} & \bf .169 & .177 & \emph{.167} & \bf .198 \\
%-0.023  SEMANTIC_ROLES                 -0.028(11594)   0.005(11934)    0.011(9796)     -0.081(11021)
%0.014   DR-QCRI-0:SEMANTIC_ROLES        0.007(11594)    0.053(11934)    0.028(9796)     -0.033(11021)
%0.176   DR-QCRI-2:SEMANTIC_ROLES        0.181(11594)    0.197(11934)    0.191(9796)     0.135(11021)
\srl & -.028 & \bf .007 & \bf .181 & .005 & \bf .053 & \bf .197 & .011 & \bf .028 & \bf .191 & -.081 & \bf -.033 & \bf .135 & -.023 & \bf .014 & \bf .176 \\
%0.134   DISCOURSE               0.138(11594)    0.122(11934)    0.161(9796)     0.113(11021)
%0.147   DR-QCRI-0:DISCOURSE     0.151(11594)    0.144(11934)    0.168(9796)     0.125(11021)
%0.203   DR-QCRI-2:DISCOURSE     0.209(11594)    0.201(11934)    0.214(9796)     0.188(11021)
\dis & .138 & \bf .151 & \bf .209 & .122 & \bf .144 & \bf .201 & .161 & \bf .168 & \bf .214 & .113 & \bf .125 & \bf .188 & .134 & \bf .147 & \bf .203 \\
%0.254   2009            0.254(11594)    0.287(11934)    0.264(9796)     0.212(11021)
%0.249   DR-QCRI-0:2009  0.253(11594)    0.273(11934)    0.264(9796)     0.206(11021)
%0.260   DR-QCRI-2:2009  0.259(11594)    0.293(11934)    0.266(9796)     0.221(11021)
\asiyaix & .254 & \emph{.253} & \bf .259 & .287 & \emph{.273} & \bf .293 & .264 & .264 & \bf .266 & .212 & \emph{.206} & \bf .221 & .254 & \emph{.249} & \bf .260 \\
%0.268   ALL             0.263(11594)    0.305(11934)    0.269(9796)     0.235(11021)
%0.263   DR-QCRI-0:ALL   0.263(11594)    0.288(11934)    0.272(9796)     0.229(11021)
%0.270   DR-QCRI-2:ALL   0.269(11594)    0.303(11934)    0.269(9796)     0.239(11021)
\asiyaall & .263 & .263 & \bf .269 & .305 & \emph{.288} & \emph{.303} & .269 & \bf .272 & .269 & .235 & \emph{.229} & \bf .239 & .268 & \emph{.263} & \bf .270 \\
\hline
AVERAGE & .170 & .150 & .212 & .181 & .155 & .209 & .174 & .153 & .213 & .134 & .106 & .171 & .165 & .141 & .201\\
diff & & -.020 & +.042 &  & -.026 & +.028 &  & -.020 & +.039 &  & -.028 & +.037 &  & -.024 & +.037\\
\hline
\end{tabular}}
\end{center}
\caption{\label{tab:results-wmt12-seg}Results on WMT12 at the segment level. Kendall's Tau with human judgments.}
\end{table*}



%--------------------------------
\subsection{System-level Results}

Table~\ref{tab:results-wmt12-sys} shows the system-level experimental results for WMT12.
We follow the evaluation setup of the metrics task of WMT12 \cite{WMT12},
and we use the official script from WMT2012 to calculate the Pearson correlation
(where higher \emph{absolute} values indicate better metrics performance)
with human pairwise judgments
collected for the systems that participated in the metrics task.
We only consider translation into English,
for which segment-level judgments are available for four language pairs:
Czech-English (cs-en, 6 systems),
German-English (de-en, 16 systems),
Spanish-English (es-en, 12 systems),
and
French-English (fr-en, 15 systems).
We present the results for the individual language pairs as well as the average over all four. %languages.
These results are grouped into four groups in Table~\ref{tab:results-wmt12-sys}:

Group I (lines 1-2) contains our evaluation metrics, \qcri \ and \qcril.
%%% Lluís: what if we call them "similarity measures" so as to avoid the idea that we are presenting new metrics?
%%% Preslav: I thought of this, but then -- this is a metrics task. I had it for a while different, then made it all "metrics" for consistency.

Group II (lines 3-13) includes the metrics that participated in the WMT12 metrics task,
(excluding SAGAN-STS, which did not have results for all language pairs).

Group III (lines 14-15) contains two other important evaluation metrics,
which were not considered in the WMT12 metrics task: \nist \ and \rouge.

Group IV (lines 16-21) includes the metric combinations calculated with \asiya\ and
described in Section~\ref{sec:experiments}.

For each metric in groups II, III and IV,
Table~\ref{tab:results-wmt12-sys} presents the results for the original metric
as well for the uniform linear combinations of that metric with \qcri \ and with \qcril.
The combinations with \qcri \ and \qcril \ that improve over the original metrics are
shown in \textbf{bold}, and those that degrade are in \emph{italic}.

The last two rows show
(i) the average score over all metrics, excluding \qcri \ and \qcril,
and
(ii) the differences in the correlations for the \qcri/\qcril-combined and the original metrics.

We can see that \qcri\ is weak by itself: on the average, it has a correlation of .592,
while the metrics from group II score from .735 to .902.
This performance of \qcri \ is to be expected as it is completely unlexicalized, and thus it misses important cues.
However, overall, \qcri \ yields improvements when combined with 15 of the 19 metrics in Table~\ref{tab:results-wmt12-sys};
it also leaves one metric unchanged, worsening only three of the metrics.
This suggests that \qcri \ contains information that is complementary to that used by the other metrics.
Note that this is true both for the individual metrics from groups II and III
as well as for the metric combinations in group IV.
These combinations involve several metrics using linguistic information at different levels and
thus are hard to improve over; yet, \qcri \ does improve, which suggests that it has something
complementary to offer. Note also that all combinations here are untuned -- they are simple
linear combinations, where all metrics get equal weights.

% Preslav: I am speculating here... Please, check!
% Lluís: fine with me for the first part; Shafiq should check that the claim on the parser "failure" for cs-en is true
Looking at the individual languages,
we can see that the combination with \qcri \  works best for de-en and fr-en,
but has hard time improving cs-en.
We believe that the low performance for cs-en is due to \qcri \ being too weak as an individual metric for this language pair
(e.g., because of low quality translations, which are hard to parse by the discourse parser);
thus, it has little to offer.
For \hbox{es-en}, the combination hurts for only one metric,
but it also leaves most of 11 of the 19 metrics without changes.
We explain the failure to improve by the higher performance of the original metrics for this language pair,
which leaves very little space for improvement (but there is also no decrease!).
Overall, combining the metrics with \qcri \ yields quite sizable correlation improvements for three of
the four language pairs:
+.022 for de-en,
+.014 for es-en,
and
+.010 for fr-en.
%However, it hurts for cs-en,
%and thus the net overall improvement is +.007 on the average.

% Preslav: Some speculation below, check!
% Lluís: I don't see we can say anything much different; This is the most annoying point of the paper: DR-ex works doesn't work at all at system level even though individually it is better than DR, which does help! We may add that this point requires further research. It is a pity that we have to start the analysis by this table, which is the less convincing.
Let us now have a look at \qcril. Naturally, it performs better than \qcri \ since it is lexicalized.
Individually, it outperforms three of the metrics from group II for fr-en,
five of the metrics from group II for de-en,
and all metrics (from all groups!) for es-en.
However, it performs very poorly on cs-en,
and thus, it cannot outperform any of the individual metrics in Table~\ref{tab:results-wmt12-sys} on its own.
Interestingly, even though it is much better than \qcri,
\qcril \ fails to yield improvements when combined with most of the metrics:
it only improves over the last two metrics from group IV.
We believe this is because the way \qcril \ uses lexical information is somewhat weak compared to other metrics.
Thus, it is better to combine with \qcri, which is unlexicalized and only uses discourse structure.

Overall, we can conclude that at the system level,
combining a metric with \qcri \ is a good idea for most of the metrics.
\qcril \ is stronger individually, but is not as good for combinations.

\vspace{-1mm}
%--------------------------------------------
\subsection{Segment-level Results: Non-tuned}

Table~\ref{tab:results-wmt12-seg} shows the results for WMT12 at the segment level.
Following, the WMT12 metrics task evaluation setup, we use Kendall's Tau for scoring.
Note that it can take both positive and negative values,
and unlike Pearson's correlation where the sign did not matter,
here negative values are worse than positive ones.\footnote{We have fixed a bug in the scoring tool from WMT12,
which was making all scores positive.
This made \terrorcat's score negative, as we present it in Table~\ref{tab:results-wmt12-seg}.}
Table~\ref{tab:results-wmt12-seg} has the same structure as Table~\ref{tab:results-wmt12-sys},
and it groups the results in the same four groups,
but this time some of the metrics in groups II and III are different
since the set of participating systems differed between the segment and the system level.

We can see in Table~\ref{tab:results-wmt12-seg}
that \qcri \ is very bad as an individual metric, with a high negative score of -.422.
This should not be surprising:
the discourse parse tree clearly does not contain enough information for good evaluation at the segment level.
This was not that much of a problem at the system level, where evidence from all 3,003 test sentences was accumulated,
but it is a problem when a good score is to be derived from a single discourse parse tree,
which can be also wrong or void.
Due to the low score of \qcri \ as an individual metric,
it fails to yield improvements when combined with other metrics
except for the three worst metrics. This is consistent for all language pairs.

Again, \qcril \ is better than \qcri; in fact, it is much better, with a positive Tau of +.165.
As an individual metric, it ranks exactly in the middle of the metrics that participated in WMT12 for
the segment level.
When linearly combined with other metrics, \qcril \ outperforms 15 of the 19 in Table~\ref{tab:results-wmt12-seg},
and it matches the score of another metric, only losing to the top three metrics from group II.
On the average, \qcril \ yields +.037 Tau of absolute improvement across all metrics,
i.e., from .165 to .201; the improvement is very similar across all languages.
This is large improvement, taking into account that the combinations are not tuned.

\vspace{-1mm}
%----------------------------------------
\subsection{Segment-level Results: Tuned}

Next, we experimented with tuning the weights of the individual metrics in the metric combinations,
using the learning method described in Section~\ref{DataPreprocess}.
We did this using cross-validation on WMT12. We used ten folds of approximately equal sizes,
each containing about 300 sentences: we constructed the folds by putting together entire documents,
thus not allowing sentences from a document to be split over two different folds.
We then trained on all human WMT12 judgments for all systems that are about the sentences from the
training folds, putting all language pairs together.\footnote{Tuning separately
for each language pair yielded slightly lower results.}

The results are shown in Table~\ref{tab:results-wmt12-seg-tuned}.
To save space, we only show the average over the four language pairs,
but the results are similar across all the language pairs.
We can see that the tuned combinations with \qcril \ improve over all 19 original metrics,
including the top three best-performing ones from group II.
Interestingly, the tuned combinations with the much weaker metric \qcri \ now improve over 18 of the original metrics,
and match the score of the 19th one.
On the average, \qcri \ improves Tau from .165 to .201, which is +.036,
while \qcril \ improves to .231 (or +.066).

Note that the \asiya\ metrics are combining several metrics, and these combinations (which exclude \qcri \ and \qcril)
can be also tuned;
this yields sizable improvements over the untuned versions as column three in the table shows.
Compared to this baseline, \qcri \ improves for three of the six \asiya\ metrics,
while \qcril \ improves for five and matches the score of the sixth one.
Note that improving over the last two \asiya\ metrics is very hard:
they have very high scores of .297 and .295;
for comparison, the best segment-level system at WMT12 (\spede) achieved a Tau of .254.

In order to rule out the possibility that the improvement of the tuned metrics on WMT12 comes from overfitting
and the tuned metrics do not really generalize when applied to other sentences, we also tested on a fresh test set: WMT11.
I.e., we tuned the weights on \emph{all} WMT12 pairwise judgments (no cross-validation), and we tested on WMT11.
The results are shown in Table~\ref{tab:results-wmt11-seg-tuned}.
Since the systems that participated in WMT11 and WMT12 are different
(and even when they have the same name, there is no guarantee that they have not changed from 2011 to 2012),
we only report results for \nist, \rouge, \ter, and \bleu, where we use the versions available in \asiya,
as well as for the \asiya\ metrics, thus making sure the metrics involved are the same for 2011 and 2012.
Once again, tuning yields sizable improvements over the simple combination for the \asiya\ metrics,
but adding \qcril \ to the combinations manages to improve over all tuned \asiya\ metrics.
In contrast, adding \qcri \ only improves for three of the six tuned \asiya\ metrics.
However, both \qcri \ and \qcril \ improve over \nist, \rouge, \ter, and \bleu.
On the average, \qcri \ improves Tau from .216 to .250, which is +.034,
while \qcril \ improves to .275 or +.059.
These improvements are very close to those for the WMT12 cross-validation.
This shows that the weights learned on WMT12 are good and do not overfit to 2012
as they are also good for WMT11.

What is interesting is that when tuning is used, \qcri \ helps achieve sizeable improvements,
even if not as strong as for \qcril. This is remarkable given that \qcri \ has a strong negative
Tau as an individual metric at the sentence level. This suggests that both \qcri \ and \qcril \
contain information that is complementary to that of the individual metrics that we experimented with.

Overall, from the experimental results in this section, we can conclude that discourse structure
is an important information source to be taken into account in the automatic evaluation of machine
translation output.


% Preslav: I have written the text below and then I have removed it. In fact, we can tune a metric at the system level too!
% Preslav: We have absolute human scores for the systems: we can use these scores to induce pairwise judgments between systems.
% Preslav: Or we can try to learn to predict them as a regression task -- OK, food for thought for future work...

%Note that we could not do tuned combination experiments for the system-level evaluation
%because we do not have pairwise human judgments for the systems: we only have scores.
%One might think that we could use the combination weights learned at the segment level
%to combine metrics at the system level.
%The problem is that the metrics that participated in the segment-level and the system-level tracks of WMT12 are different.
%Even when they have the same name, they are calculated differently,
%and, for most metrics, we cannot obtain the system-level score as a combination of segment-level scores.
%For example, \bleu \ calculates a global brevity penalty, which is not expressible as a function of the brevity penalties
%of the individual segments. The problem remains even if we try to obtain system-level scores from fold-level scores.
%If we tune with say \bleu+\qcri at the segment level,
%the learned weights would not be adequate for \bleu+\qcri at the system level
%because \bleu \ will be calculated differently.
%More importantly, the evaluation measure for segment-level and system-level metrics is different too:
%Kendall's Tau vs. Person correlation.
%Thus, it does not make sense to optimize one measure and then be tested on a different one.
%Given all these issues, we report no tuned system-level results.



\begin{table}[t]
\begin{center}
{\small\begin{tabular}{r|r|rrr|}
\cline{2-5}
& Orig. & \multicolumn{3}{|c|}{Tuned}\\
\cline{2-5}
Metrics &  & & +\sqcri & +\sqcril\\
\hline
%-0.422  DR-QCRI-0
\qcri & -.422 & -- & -- & --\\
%0.165   DR-QCRI-2
\qcril & .165 & -- & -- & -- \\
\hline
%0.254   spede07_pP                      0.260(11594)    0.278(11934)    0.265(9796)     0.212(11021)
%0.174   DR-QCRI-0:spede07_pP_norm       0.185(11594)    0.186(11934)    0.195(9796)     0.132(11021)
%0.225   DR-QCRI-2:spede07_pP_norm       0.232(11594)    0.229(11934)    0.246(9796)     0.192(11021)
%0.254   DR-QCRI-spede07_pP_dr   0.260(11594)    0.280(11934)    0.266(9796)     0.209(11021)
%0.256   DR-QCRI-spede07_pP_dr_l 0.262(11594)    0.279(11934)    0.264(9796)     0.220(11021)
\spede & .254 & -- & .254 & \bf .256\\
%0.247   Meteor                  0.251(11594)    0.275(11934)    0.249(9796)     0.212(11021)
%0.173   DR-QCRI-0:Meteor_norm   0.183(11594)    0.186(11934)    0.185(9796)     0.140(11021)
%0.232   DR-QCRI-2:Meteor_norm   0.241(11594)    0.243(11934)    0.243(9796)     0.202(11021)
%0.250   DR-QCRI-Meteor_dr       0.250(11594)    0.278(11934)    0.257(9796)     0.214(11021)
%0.251   DR-QCRI-Meteor_dr_l     0.259(11594)    0.278(11934)    0.253(9796)     0.215(11021)
\meteor & .247 & -- & \bf .250 & \bf .251\\
%0.229   AMBER                   0.245(11594)    0.248(11934)    0.231(9796)     0.191(11021)
%0.178   DR-QCRI-0:AMBER_norm    0.201(11594)    0.189(11934)    0.186(9796)     0.137(11021)
%0.224   DR-QCRI-2:AMBER_norm    0.238(11594)    0.233(11934)    0.231(9796)     0.195(11021)
%0.230   DR-QCRI-AMBER_dr        0.249(11594)    0.252(11934)    0.229(9796)     0.191(11021)
%0.231   DR-QCRI-AMBER_dr_l      0.245(11594)    0.242(11934)    0.237(9796)     0.201(11021)
\amber & .229 & -- & \bf .230 & \bf .231 \\
%0.172   SIMPBLEU                0.193(11594)    0.172(11934)    0.189(9796)     0.134(11021)
%0.133   DR-QCRI-0:SIMPBLEU_norm 0.153(11594)    0.142(11934)    0.149(9796)     0.088(11021)
%0.208   DR-QCRI-2:SIMPBLEU_norm 0.226(11594)    0.206(11934)    0.223(9796)     0.177(11021)
%0.181   DR-QCRI-SIMPBLEU_dr     0.202(11594)    0.190(11934)    0.189(9796)     0.144(11021)
%0.206   DR-QCRI-SIMPBLEU_dr_l   0.224(11594)    0.211(11934)    0.222(9796)     0.169(11021)
\simpbleu &  .172 & -- & \bf .181 & \bf .206 \\
%-0.186  TerrorCat                       -0.178(11594)   -0.195(11934)   -0.184(9796)    -0.186(11021)
%-0.115  DR-QCRI-0:TerrorCat_norm        -0.108(11594)   -0.099(11934)   -0.111(9796)    -0.141(11021)
%-0.084  DR-QCRI-2:TerrorCat_norm        -0.041(11594)   -0.096(11934)   -0.088(9796)    -0.112(11021)
%0.181   DR-QCRI-TerrorCat_dr    0.175(11594)    0.194(11934)    0.187(9796)     0.168(11021)
%0.215   DR-QCRI-TerrorCat_dr_l  0.216(11594)    0.225(11934)    0.220(9796)     0.199(11021)
\terrorcat & -.186 & -- & \bf .181 & \bf .215\\
%0.165   XEnErrCats                      0.174(11594)    0.184(11934)    0.177(9796)     0.127(11021)
%0.127   DR-QCRI-0:XEnErrCat_norm        0.141(11594)    0.139(11934)    0.141(9796)     0.087(11021)
%0.196   DR-QCRI-2:XEnErrCat_norm        0.210(11594)    0.191(11934)    0.208(9796)     0.174(11021)
%0.175   DR-QCRI-XEnErrCats_dr   0.178(11594)    0.195(11934)    0.188(9796)     0.139(11021)
%0.195   DR-QCRI-XEnErrCats_dr_l 0.208(11594)    0.190(11934)    0.208(9796)     0.175(11021)
\xen & .165 & -- & \bf .175 & \bf .195 \\
%0.154   posF                    0.158(11594)    0.185(11934)    0.152(9796)     0.122(11021)
%0.122   DR-QCRI-0:posF_norm     0.123(11594)    0.142(11934)    0.140(9796)     0.084(11021)
%0.210   DR-QCRI-2:posF_norm     0.223(11594)    0.223(11934)    0.219(9796)     0.173(11021)
%0.160   DR-QCRI-posF_dr 0.164(11594)    0.189(11934)    0.165(9796)     0.123(11021)
%0.211   DR-QCRI-posF_dr_l       0.225(11594)    0.225(11934)    0.223(9796)     0.171(11021)
\posf & .154 & -- & \bf .160 & \bf .211\\
%0.153   WordBlockErrCats                0.152(11594)    0.161(11934)    0.168(9796)     0.130(11021)
%0.118   DR-QCRI-0:WordBlockErrCats_norm 0.126(11594)    0.119(11934)    0.134(9796)     0.092(11021)
%0.199   DR-QCRI-2:WordBlockErrCats_norm 0.206(11594)    0.203(11934)    0.218(9796)     0.168(11021)
%0.162   DR-QCRI-WrdBlkErrCats_dr        0.161(11594)    0.174(11934)    0.176(9796)     0.137(11021)
%0.198   DR-QCRI-WrdBlkErrCats_dr_l      0.206(11594)    0.201(11934)    0.218(9796)     0.168(11021)
\word & .153 & -- & \bf .162 & \bf .198\\
%0.074   BlockErrCats                    0.068(11594)    0.082(11934)    0.084(9796)     0.063(11021)
%0.062   DR-QCRI-0:BlockErrCats_norm     0.057(11594)    0.072(11934)    0.073(9796)     0.046(11021)
%0.173   DR-QCRI-2:BlockErrCats_norm     0.177(11594)    0.172(11934)    0.191(9796)     0.153(11021)
%0.088   DR-QCRI-BlkErrCats_dr   0.077(11594)    0.103(11934)    0.095(9796)     0.077(11021)
%0.183   DR-QCRI-BlkErrCats_dr_l 0.191(11594)    0.174(11934)    0.205(9796)     0.163(11021)
\block & .074 & -- & \bf .088 & \bf .183\\
\hline
%0.214   NIST            0.222(11594)    0.232(11934)    0.205(9796)     0.197(11021)
%0.168   DR-QCRI-0:NIST  0.184(11594)    0.182(11934)    0.166(9796)     0.141(11021)
%0.214   DR-QCRI-2:NIST  0.228(11594)    0.220(11934)    0.219(9796)     0.189(11021)
%0.222   DR-QCRI-NIST_dr 0.234(11594)    0.241(11934)    0.214(9796)     0.200(11021)
%0.228   DR-QCRI-NIST_dr_l       0.241(11594)    0.238(11934)    0.226(9796)     0.205(11021)
\nist & .214 & -- & \bf .222 & \bf .228\\
%0.185   ROUGE-W                 0.205(11594)    0.186(11934)    0.197(9796)     0.151(11021)
%0.136   DR-QCRI-0:ROUGE-W       0.156(11594)    0.138(11934)    0.154(9796)     0.097(11021)
%0.211   DR-QCRI-2:ROUGE-W       0.230(11594)    0.207(11934)    0.228(9796)     0.180(11021)
%0.196   DR-QCRI-ROUGE-W_dr      0.212(11594)    0.199(11934)    0.211(9796)     0.161(11021)
%0.226   DR-QCRI-ROUGE-W_dr_l    0.250(11594)    0.223(11934)    0.237(9796)     0.193(11021)
\rouge & .185 & -- & \bf .196 & \bf .226\\
%0.218   TERp-A                  0.209(11594)    0.254(11934)    0.229(9796)     0.178(11021)
%0.177   DR-QCRI-0:TERp-A        0.185(11594)    0.202(11934)    0.185(9796)     0.135(11021)
%0.244   DR-QCRI-2:TERp-A        0.240(11594)    0.264(11934)    0.269(9796)     0.204(11021)
%0.230   DR-QCRI-TERp-A_dr       0.226(11594)    0.264(11934)    0.239(9796)     0.190(11021)
%0.253   DR-QCRI-TERp-A_dr_l     0.250(11594)    0.276(11934)    0.268(9796)     0.219(11021)
\ter & .218 & -- & \bf .230 & \bf .253\\
%0.185   BLEU            0.209(11594)    0.186(11934)    0.186(9796)     0.159(11021)
%0.149   DR-QCRI-0:BLEU  0.172(11594)    0.152(11934)    0.160(9796)     0.111(11021)
%0.206   DR-QCRI-2:BLEU  0.232(11594)    0.198(11934)    0.216(9796)     0.178(11021)
%0.189   DR-QCRI-BLEU_dr 0.214(11594)    0.191(11934)    0.192(9796)     0.159(11021)
%0.206   DR-QCRI-BLEU_dr_l       0.231(11594)    0.197(11934)    0.216(9796)     0.179(11021)
\bleu & .185 & -- & \bf .189 & \bf .206\\
\hline

%0.254   LEXICAL                 0.258(11594)    0.277(11934)    0.258(9796)     0.224(11021)
%0.235   DR-QCRI-0:LEXICAL       0.244(11594)    0.252(11934)    0.244(9796)     0.201(11021)
%0.257   DR-QCRI-2:LEXICAL       0.264(11594)    0.272(11934)    0.267(9796)     0.225(11021)
%0.266   DR-QCRI-LEX     0.266(11594)    0.288(11934)    0.277(9796)     0.231(11021)
%0.268   DR-QCRI-LEX_dr  0.272(11594)    0.292(11934)    0.278(9796)     0.230(11021)
%0.270   DR-QCRI-LEX_dr_l        0.274(11594)    0.291(11934)    0.280(9796)     0.233(11021)
\lex & .254 & .266 & \bf .268 & \bf .270 \\
%0.177   PARSING                 0.186(11594)    0.189(11934)    0.186(9796)     0.149(11021)
%0.167   DR-QCRI-0:PARSING       0.177(11594)    0.179(11934)    0.183(9796)     0.129(11021)
%0.198   DR-QCRI-2:PARSING       0.206(11594)    0.207(11934)    0.211(9796)     0.169(11021)
%0.228   DR-QCRI-SYN     0.229(11594)    0.266(11934)    0.232(9796)     0.186(11021)
%0.228   DR-QCRI-SYN_dr  0.229(11594)    0.265(11934)    0.233(9796)     0.183(11021)
%0.243   DR-QCRI-SYN_dr_l        0.238(11594)    0.267(11934)    0.262(9796)     0.206(11021)
\syn & .177 & .228 & .228 & \bf .243 \\
%-0.023  SEMANTIC_ROLES                 -0.028(11594)   0.005(11934)    0.011(9796)     -0.081(11021)
%0.014   DR-QCRI-0:SEMANTIC_ROLES        0.007(11594)    0.053(11934)    0.028(9796)     -0.033(11021)
%0.176   DR-QCRI-2:SEMANTIC_ROLES        0.181(11594)    0.197(11934)    0.191(9796)     0.135(11021)
%-0.002  DR-QCRI-SRL     -0.008(11594)   0.023(11934)    0.033(9796)     -0.057(11021)
%0.040   DR-QCRI-SRL_dr  0.036(11594)    0.081(11934)    0.057(9796)     -0.012(11021)
%0.211   DR-QCRI-SRL_dr_l        0.216(11594)    0.222(11934)    0.224(9796)     0.183(11021)
\srl & -.023 & -.002 & \bf .040 & \bf .211 \\
%0.134   DISCOURSE               0.138(11594)    0.122(11934)    0.161(9796)     0.113(11021)
%0.147   DR-QCRI-0:DISCOURSE     0.151(11594)    0.144(11934)    0.168(9796)     0.125(11021)
%0.203   DR-QCRI-2:DISCOURSE     0.209(11594)    0.201(11934)    0.214(9796)     0.188(11021)
%0.147   DR-QCRI-DIS     0.155(11594)    0.136(11934)    0.174(9796)     0.123(11021)
%0.176   DR-QCRI-DIS_dr  0.196(11594)    0.163(11934)    0.196(9796)     0.151(11021)
%0.211   DR-QCRI-DIS_dr_l        0.217(11594)    0.208(11934)    0.227(9796)     0.193(11021)
\dis & .134 & .147 & \bf .176 & \bf .211 \\
%0.254   2009            0.254(11594)    0.287(11934)    0.264(9796)     0.212(11021)
%0.249   DR-QCRI-0:2009  0.253(11594)    0.273(11934)    0.264(9796)     0.206(11021)
%0.260   DR-QCRI-2:2009  0.259(11594)    0.293(11934)    0.266(9796)     0.221(11021)
%0.296   DR-QCRI-ALL     0.291(11594)    0.328(11934)    0.304(9796)     0.260(11021)
%0.297   DR-QCRI-2009    0.298(11594)    0.327(11934)    0.301(9796)     0.261(11021)
%0.295   DR-QCRI-2009_dr 0.298(11594)    0.324(11934)    0.299(9796)     0.260(11021)
%0.297   DR-QCRI-2009_dr_l       0.296(11594)    0.325(11934)    0.305(9796)     0.261(11021)
\asiyaix & .260 & .297 & \emph{.295} & .297 \\
%0.268   ALL             0.263(11594)    0.305(11934)    0.269(9796)     0.235(11021)
%0.263   DR-QCRI-0:ALL   0.263(11594)    0.288(11934)    0.272(9796)     0.229(11021)
%0.270   DR-QCRI-2:ALL   0.269(11594)    0.303(11934)    0.269(9796)     0.239(11021)
%???? 0.296   DR-QCRI-ALL     0.291(11594)    0.328(11934)    0.304(9796)     0.260(11021)
%0.295   DR-QCRI-ULC     0.291(11594)    0.325(11934)    0.304(9796)     0.261(11021)
%0.295   DR-QCRI-ULC_dr  0.293(11594)    0.328(11934)    0.304(9796)     0.256(11021)
%0.297   DR-QCRI-ULC_dr_l        0.293(11594)    0.329(11934)    0.304(9796)     0.262(11021)
\asiyaall & .268 & .295 & .295 & \bf .297\\
\hline
AVERAGE & .165 & & .201 & .231\\
diff    &      & & +.036 & +.066\\
\hline
\end{tabular}}
\end{center}
\caption{\label{tab:results-wmt12-seg-tuned}Averaged results on WMT12 at the segment level: tuning with cross-validation on WMT12. Kendall's Tau with human judgments.}
\end{table}

%\begin{table*}[t]
%\begin{center}
%{\small\begin{tabular}{r|rrr|rrr|rrr|rrr|rrr|}
%\cline{2-7}
%& \multicolumn{3}{|c|}{Simple AVG} & \multicolumn{3}{|c|}{Weighted AVG}\\
%\cline{2-7}
%Metrics &  & +\sqcri & +\sqcril &  & +\sqcri & +\sqcril\\
%\hline
%\qcri & .257 & -- & -- & -- & -- & --\\
%\qcril & .371 & -- & -- & -- & -- & --\\
%\hline
%%0.902   SEMPOS                  0.943   0.924   0.937   0.804
%%0.897   DR-QCRI-0:SEMPOS_norm   0.886   0.924   0.937   0.843
%%0.826   DR-QCRI-2:SEMPOS_norm   0.714   0.874   0.923   0.793
%\sempos & .902 & \emph{.897} & \emph{.826} & -- & ? & ?\\
%%0.857   AMBER                   0.829   0.785   0.965   0.85
%%0.869   DR-QCRI-0:AMBER_norm    0.829   0.835   0.979   0.832
%%0.775   DR-QCRI-2:AMBER_norm    0.657   0.75    0.916   0.779
%%0.847   DR-QCRI-AMBER_dr        0.829   0.835   0.965   0.757
%%0.830   DR-QCRI-AMBER_dr_l      0.829   0.838   0.93    0.721
%\amber & .857 & \bf .869 & \emph{.775} & -- & \emph{.847} & \emph{.830}\\
%%0.834   Meteor                  0.657   0.885   0.951   0.843
%%0.840   DR-QCRI-0:Meteor_norm   0.6     0.912   0.986   0.861
%%0.760   DR-QCRI-2:Meteor_norm   0.6     0.762   0.916   0.761
%%0.835   DR-QCRI-Meteor_dr       0.657   0.918   0.916   0.85
%%0.775   DR-QCRI-Meteor_dr_l     0.657   0.874   0.832   0.736
%\meteor & .834 & \bf .840 & .760 & -- & \bf .835 & \emph{.775}\\
%%0.831   TerrorCat                        0.714   0.762   0.965   0.882
%%0.786   DR-QCRI-0:TerrorCat_norm        -0.886  -0.476  -0.951  -0.832
%%0.538   DR-QCRI-2:TerrorCat_sum         -0.657  -0.126  -0.580  -0.789
%%0.833   DR-QCRI-TerrorCat_dr    0.714   0.771   0.965   0.882
%%0.700   DR-QCRI-TerrorCat_dr_l  0.6     0.715   0.741   0.743
%\terrorcat & .831 & \emph{.786} & \emph{.538} & -- & \bf .833 & \emph{.700}\\
%%0.823   SIMPBLEU                        0.886   0.697   0.888   0.821
%%0.832   DR-QCRI-0:SIMPBLEU_norm         0.829   0.765   0.902   0.832
%%0.741   DR-QCRI-2:SIMPBLEU_norm         0.657   0.621   0.881   0.807
%%0.822   DR-QCRI-SIMPBLEU_dr     0.829   0.768   0.888   0.804
%%0.698   DR-QCRI-SIMPBLEU_dr_l   0.543   0.709   0.804   0.736
%\simpbleu & .823 & \bf .832 & \emph{.741} & -- & \emph{.822} & \emph{.698}\\
%%0.812   TER                    -0.886  -0.624  -0.916  -0.821
%%0.844   DR-QCRI-0:TER_norm      0.886   0.709   0.951   0.829
%%0.795   DR-QCRI-2:TER_norm      0.829   0.609   0.923   0.818
%%0.902   DR-QCRI-TERp-A_dr       0.943   0.835   0.972   0.857
%%0.801   DR-QCRI-TERp-A_dr_l     0.6     0.832   0.951   0.821
%\ter & .812 & \bf .844 & \emph{.795} & -- & \bf .902* & \emph{.801}*\\
%%0.810   BLEU_4_closest_cased                    0.886   0.671   0.874   0.811
%%0.822   DR-QCRI-0:BLEU_4_closest_cased_norm     0.886   0.679   0.895   0.829
%%0.783   DR-QCRI-2:BLEU_4_closest_cased_norm     0.829   0.618   0.881   0.804
%%0.846   DR-QCRI-BLEU_dr         0.943   0.724   0.895   0.821
%%0.715   DR-QCRI-BLEU_dr_l       0.543   0.676   0.874   0.768
%\bleu & .810 & \bf .822 & \emph{.783} & -- & \bf .846* & \emph{.715}*\\
%%0.754   posF                    0.657   0.662   0.874   0.825
%%0.767   DR-QCRI-0:posF_norm     0.543   0.774   0.881   0.871
%%0.696   DR-QCRI-2:posF_sum      0.543   0.624   0.846   0.771
%%0.751   DR-QCRI-posF_dr         0.6     0.721   0.853   0.832
%%0.668   DR-QCRI-posF_dr_l       0.543   0.724   0.734   0.671
%\posf & .754 & \bf .767 & \emph{.696} & -- & \bf .751 & \emph{.668}\\
%%0.751   BlockErrCats                   -0.638  -0.747  -0.881  -0.738
%%0.749   DR-QCRI-0:BlockErrCats_norm     0.6     0.771   0.881   0.746
%%0.740   DR-QCRI-2:BlockErrCats_norm     0.6     0.741   0.874   0.746
%%0.755   DR-QCRI-BlkErrCats_dr   0.6     0.768   0.881   0.771
%%0.658   DR-QCRI-BlkErrCats_dr_l         0.543   0.724   0.734   0.632
%\sblock & .751 & \emph{.749} & \emph{.740} & -- & \bf .755 & \emph{.658}\\
%%0.738   WordBlockErrCats                       -0.657  -0.674  -0.853  -0.768
%%0.752   DR-QCRI-0:WordBlockErrCats_norm         0.657   0.709   0.853   0.789
%%0.709   DR-QCRI-2:WordBlockErrCats_norm         0.6     0.685   0.846   0.704
%%0.733   DR-QCRI-WrdBlkErrCats_dr        0.6     0.668   0.867   0.796
%%0.669   DR-QCRI-WrdBlkErrCats_dr_l      0.543   0.682   0.776   0.675
%\sword & .738 & \bf .752 & \emph{.709} & -- & \emph{.733} & \emph{.669}\\
%%0.735   XEnErrCats                     -0.657  -0.638  -0.874  -0.771
%%0.743   DR-QCRI-0:XEnErrCats_norm       0.657   0.662   0.874   0.779
%%0.725   DR-QCRI-2:XEnErrCats_norm       0.657   0.618   0.846   0.779
%%0.750   DR-QCRI-XEnErrCats_dr   0.657   0.665   0.881   0.796
%%0.673   DR-QCRI-XEnErrCats_dr_l         0.543   0.659   0.804   0.686
%\sxen & .735 & \bf .743 & \emph{.725} & -- & \bf .750 & \emph{.673}\\
%\hline
%%0.817   NIST            0.943   0.682   0.832   0.811
%%0.864   DR-QCRI-0:NIST  0.886   0.75    0.979   0.839
%%0.763   DR-QCRI-2:NIST  0.657   0.644   0.923   0.829
%%0.883   DR-QCRI-NIST_dr         1.0     0.782   0.93    0.818
%%0.870   DR-QCRI-NIST_dr_l       0.943   0.774   0.958   0.804
%\nist & .817 & \bf .864 & \emph{.763} & -- & \bf .883 & \bf .870\\
%%0.884   ROUGE-W                 1.0     0.765   0.965   0.807
%%0.887   DR-QCRI-0:ROUGE-W       0.886   0.859   0.965   0.839
%%0.767   DR-QCRI-2:ROUGE-W       0.6     0.756   0.923   0.789
%\rouge & .884 & \bf .887 & \emph{.767} \\
%\hline
%%0.876   LEXICAL                 0.943   0.776   0.944   0.843
%%0.876   DR-QCRI-0:LEXICAL       0.943   0.776   0.944   0.843
%%0.870   DR-QCRI-2:LEXICAL       0.943   0.768   0.93    0.839
%\lex & .876 & .876 & \emph{.870} \\
%%0.893   PARSING                 0.943   0.903   0.902   0.825
%%0.899   DR-QCRI-0:PARSING       0.943   0.918   0.902   0.832
%%0.878   DR-QCRI-2:PARSING       0.886   0.894   0.902   0.829
%\syn & .893 & \bf .899 & \emph{.878} \\
%%0.910   SEMANTIC_ROLES                  0.943   0.888   0.965   0.843
%%0.913   DR-QCRI-0:SEMANTIC_ROLES        0.943   0.9     0.965   0.843
%%0.906   DR-QCRI-2:SEMANTIC_ROLES        0.943   0.891   0.965   0.825
%\srl & .910 & \bf .913 & \emph{.906} \\
%%0.893   DISCOURSE               0.886   0.894   0.93    0.861
%%0.896   DR-QCRI-0:DISCOURSE     0.886   0.897   0.93    0.871
%%0.838   DR-QCRI-2:DISCOURSE     0.714   0.865   0.93    0.843
%\dis & .893 & \bf .896 & \emph{.838} \\
%%0.905   ULC2                    0.943   0.891   0.951   0.836
%%0.909   DR-QCRI-0:ULC2          0.943   0.906   0.951   0.836
%%0.909   ALL2009-DR-QCRI-2       0.943   0.891   0.951   0.85
%2009 & .905 & \bf .909 & \bf .909 \\
%%0.886   ULC             0.943   0.821   0.944   0.836
%%0.900   DR-QCRI-0:ULC   0.943   0.879   0.944   0.836
%%0.891   ALL-DR-QCRI-2   0.943   0.826   0.944   0.85
%\ulc & .886 & \bf .900 & \bf .891 \\
%\hline
%AVERAGE \\
%diff \\
%\hline
%\end{tabular}}
%\end{center}
%\label{tab:results-wmt12-sys}
%\caption{Tuned vs. non-tuned results on the WMT12 corpus at the system level (averaged over all languages).
%         Pearson correlation with human judgments.}
%\end{table*}

\begin{table}[t]
\begin{center}
{\small\begin{tabular}{r|r|rrr|}
\cline{2-5}
& Orig. & \multicolumn{3}{|c|}{Tuned}\\
\cline{2-5}
Metrics &  & & +\sqcri & +\sqcril\\
\hline
%-0.424  DR-QCRI-0       -0.454(6337)    -0.398(8950)    -0.420(5974)    -0.424(3695)
\qcri & -.424 & -- & -- & --\\
%0.176   DR-QCRI-2       0.143(6337)     0.129(8950)     0.213(5974)     0.218(3695)
\qcril & .176 & -- & -- & -- \\
\hline
%0.219   NIST    0.187(6337)     0.163(8950)     0.295(5974)     0.231(3695)
%0.228   DR-QCRI-NIST_dr 0.199(6337)     0.169(8950)     0.296(5974)     0.247(3695)
%0.230   DR-QCRI-NIST_dr_l       0.196(6337)     0.177(8950)     0.301(5974)     0.244(3695)
\nist & .219 & -- & \bf .228 & \bf .230 \\
%0.205   ROUGE-W 0.177(6337)     0.132(8950)     0.281(5974)     0.231(3695)
%0.221   DR-QCRI-RG_dr   0.186(6337)     0.154(8950)     0.281(5974)     0.264(3695)
%0.243   DR-QCRI-RG_dr_l 0.201(6337)     0.178(8950)     0.305(5974)     0.288(3695)
\rouge & .205 & -- & \bf .221 & \bf .243 \\
%0.262   TERp-A  0.233(6337)     0.210(8950)     0.331(5974)     0.275(3695)
%0.274   DR-QCRI-TER_dr  0.245(6337)     0.223(8950)     0.342(5974)     0.287(3695)
%0.291   DR-QCRI-TER_dr_l        0.258(6337)     0.239(8950)     0.360(5974)     0.306(3695)
\ter & .262 & -- & \bf .274 & \bf .291 \\
%0.186   BLEU    0.157(6337)     0.130(8950)     0.249(5974)     0.208(3695)
%0.196   DR-QCRI-BL_dr   0.168(6337)     0.140(8950)     0.251(5974)     0.223(3695)
%0.215   DR-QCRI-BL_dr_l 0.183(6337)     0.150(8950)     0.286(5974)     0.241(3695)
\bleu & .186 & -- & \bf .196 & \bf .215 \\
\hline
%0.281   LEXICAL 0.244(6337)     0.230(8950)     0.352(5974)     0.300(3695)
%0.262   DR-QCRI-0:LEXICAL       0.221(6337)     0.211(8950)     0.324(5974)     0.294(3695)
%0.282   DR-QCRI-2:LEXICAL       0.239(6337)     0.222(8950)     0.353(5974)     0.314(3695)
%tuned:
%0.302   DR-QCRI-LEX     0.266(6337)     0.244(8950)     0.372(5974)     0.327(3695)
%0.304   DR-QCRI-LEX_dr  0.271(6337)     0.247(8950)     0.373(5974)     0.325(3695)
%0.305   DR-QCRI-LEX_dr_l        0.267(6337)     0.246(8950)     0.378(5974)     0.327(3695)
\lex & .281 & .302 & \bf .304 & \bf .305 \\
%0.215   PARSING 0.197(6337)     0.187(8950)     0.262(5974)     0.214(3695)
%0.194   DR-QCRI-0:PARSING       0.169(6337)     0.183(8950)     0.235(5974)     0.190(3695)
%0.231   DR-QCRI-2:PARSING       0.202(6337)     0.212(8950)     0.277(5974)     0.234(3695)
%tuned:
%0.258   DR-QCRI-SYN     0.226(6337)     0.250(8950)     0.310(5974)     0.248(3695)
%0.261   DR-QCRI-SYN_dr  0.227(6337)     0.254(8950)     0.308(5974)     0.256(3695)
%0.277   DR-QCRI-SYN_dr_l        0.226(6337)     0.269(8950)     0.316(5974)     0.296(3695)
\syn & .215 & .258 & \bf .261 & \bf .277 \\
%-0.004  SEMANTIC_ROLES  0.024(6337)     -0.036(8950)    0.017(5974)     -0.023(3695)
%0.027   DR-QCRI-0:SEMANTIC_ROLES        0.034(6337)     0.013(8950)     0.031(5974)     0.029(3695)
%0.195   DR-QCRI-2:SEMANTIC_ROLES        0.176(6337)     0.178(8950)     0.219(5974)     0.209(3695)
%tuned:
%0.015   DR-QCRI-SRL     0.018(6337)     -0.036(8950)    0.069(5974)     0.009(3695)
%0.058   DR-QCRI-SRL_dr  0.047(6337)     0.018(8950)     0.091(5974)     0.077(3695)
%0.223   DR-QCRI-SRL_dr_l        0.192(6337)     0.185(8950)     0.254(5974)     0.260(3695)
\srl & -.004 & .015 & \bf .058 & \bf .223 \\
%0.189   DISCOURSE       0.178(6337)     0.141(8950)     0.241(5974)     0.196(3695)
%0.187   DR-QCRI-0:DISCOURSE     0.154(6337)     0.150(8950)     0.225(5974)     0.221(3695)
%0.258   DR-QCRI-2:DISCOURSE     0.217(6337)     0.209(8950)     0.301(5974)     0.306(3695)
%tuned:
%0.193   DR-QCRI-DIS     0.170(6337)     0.143(8950)     0.251(5974)     0.208(3695)
%0.223   DR-QCRI-DIS_dr  0.184(6337)     0.182(8950)     0.266(5974)     0.261(3695)
%0.257   DR-QCRI-DIS_dr_l        0.218(6337)     0.210(8950)     0.290(5974)     0.309(3695)
\dis & .189 & .268 & \emph{.263} & \bf .270 \\
%0.300   2009    0.274(6337)     0.269(8950)     0.353(5974)     0.306(3695)
%0.296   DR-QCRI-0:2009  0.264(6337)     0.272(8950)     0.340(5974)     0.308(3695)
%0.306   DR-QCRI-2:2009  0.274(6337)     0.275(8950)     0.356(5974)     0.320(3695)
%tuned:
%0.348   DR-QCRI-2009    0.308(6337)     0.311(8950)     0.403(5974)     0.371(3695)
%0.348   DR-QCRI-2009_dr 0.304(6337)     0.312(8950)     0.405(5974)     0.371(3695)
%0.349   DR-QCRI-2009_dr_l       0.305(6337)     0.311(8950)     0.403(5974)     0.376(3695)
\asiyaix & .300 & .348 & .348 & \bf .349 \\
%0.310   ALL     0.278(6337)     0.280(8950)     0.365(5974)     0.318(3695)
%0.305   DR-QCRI-0:ALL   0.266(6337)     0.278(8950)     0.352(5974)     0.324(3695)
%0.312   DR-QCRI-2:ALL   0.273(6337)     0.279(8950)     0.370(5974)     0.328(3695)
%tuned:
%0.349   DR-QCRI-ALL     0.302(6337)     0.310(8950)     0.407(5974)     0.378(3695)
%0.349   DR-QCRI-ULC_dr  0.302(6337)     0.310(8950)     0.405(5974)     0.376(3695)
%0.350   DR-QCRI-ULC_dr_l        0.305(6337)     0.311(8950)     0.407(5974)     0.375(3695)
\asiyaall & .310 & .349 & .349 & \bf .350\\
\hline
AVERAGE & .216 & & .250 & .275\\
diff    &      & & +.034 & +.059\\
\hline
\end{tabular}}
\end{center}
\caption{\label{tab:results-wmt11-seg-tuned}Averaged results on WMT11 at the segment level: tuning on the entire WMT12.
         Kendall's Tau with human judgments.}
\end{table}



%- 5- Results\\
%- - Non-Tuned\\
%- - - Individual Results\\
%- - - Linear Combination\\
%- - Tuned\\
%- - - WMT Metrics\\
%- - - ASIYA\\


==> setup.tex <==
%----------------------------------------
% Discourse Parsing for MT Evaluation
% Section 4: Experimental Setup
% Guzmán - Joty - Marquez - Nakov, January 2014
%----------------------------------------

%Results- 4- Experimental Setup\\
%- - Sources\\
%- - - WMT Metrics matr\\
%- - - - wmt2011\\
%- - - - wmt2012\\
%- - - ASIYA\\
%- - Data \& processing\\
%- - - Different Languages\\
%- - - Preprocessing steps\\
%- - Evaluation\\
%- - - System level eval\\
%- - - - Spearmans Rho\\
%- - - Segment level evaluation\\
%- - - - Kendalls Tau\\
%- - MaxEnt Combination\\
%- - - Discourse and Current Metrics\\
%- - - Discourse as a Metric component (ASIYA)\\

%\subsection{Sources}
In our experiments, we used the data available for the WMT12 %\footnote{http://www.statmt.org/wmt12/results.html}
and WMT11 metrics evaluation shared tasks\footnote{http://www.statmt.org/wmt\{11,12\}/results.html} for translations into English. The data included the output from the different participants to the WMT12  and WMT11 machine translation evaluation campaigns, both consisting of 3,003 sentences, for four different language pairs: Czech-English (cs-en), French-English (fr-en), German-English (de-en), and Spanish-English (es-en), as well as the English references. Furthermore, to measure the level of correlation of the metrics with the human judgements, we also used the human judgements (rankings) provided by the organizers. The judgements were performed by ranking the output of five systems chosen at random, for a particular sentence, also chosen at random. Thus, the overall coverage (i.e. the unique number of sentences that were evaluated) were only a fraction of the total. Also note that each judgement effectively constitutes 10 pairwise system rankings. The total number of judgements performed by humans can be observed in Table~\ref{tab:wmt-stats}.

\begin{table}[hbt]
\centering
\small
\begin{tabular}{@{}r|@{ }r@{ }r@{ }r@{ }c@{ }|r@{ }r@{ }r@{ }c|}
\hline
&\multicolumn{4}{c|}{\bf{WMT12}}&\multicolumn{4}{c|}{\bf{WMT11}} \\
%Lang. pair
&  systs &  ranks &  sents & judges & systs & ranks & sents &judges \\
    \hline
 \csen & 6 & 1,294 & 951 & 45& 8 & 498 &  171 & 20\\
 \deen & 16 & 1,427 & 975&47  & 20 & 924&  303& 31 \\
 \fren & 15 & 1,395 & 949& 44 & 18 & 708 &  249& 32\\
 \esen & 12 & 1,141 & 923&45 & 15 & 570 & 207 & 18\\
 \hline
\end{tabular}
\caption{\label{tab:wmt-stats} Statistics of number of systems (systs), number of judgements (ranks),  unique number of sentences (sents), and number of different judges (judges) for the different language pairs, for the human evaluation of the WMT12 and WMT11 shared tasks.}
\end{table}
\vspace{-2mm}
\subsection{MT Evaluation Metrics}
In this study, we evaluate to what extent existing evaluation metrics can benefit from additional
discourse information. To do so, we contrast different MT evaluation metrics with and without discourse
information. The evaluation metrics we used are described below.

\paragraph{Metrics from WMT12.} We used the publicly available scores of all metrics that participated in the WMT12 metrics evaluation shared task \cite{WMT12}, which were defined for the four language pairs. These include: \spede,  \amber, \meteor, \terrorcat, \simpbleu, \xen, \word, \block, and \posf.
%We excluded \sagan \cite{castillo-estrella:2012:WMT} because it did not have results for all four language pairs.

%%% Lluís: the following is redundant with what I explain in the following subsection
%In addition, we computed other important metrics: \nist \cite{Doddington:2002:AEM}, \bleu \cite{Papineni:Roukos:Ward:Zhu:2002}, \ter \cite{Snover06astudy} ~and \rouge \cite{Lin04}, which were not part of the WMT evaluation campaign, but are commonly used.

\paragraph{Metrics from \asiya.}
We used the \asiya\ toolkit for extending the set of evaluation measures
contrasted in this study. \asiya\ \cite{AsiyaPBML:2010} is a suite for MT evaluation,
which provides a large set of metrics making use of different levels of linguistic
information. We used the freely available version of \asiya\footnote{http://nlp.lsi.upc.edu/asiya/}
to calculate all basic metric scores and untuned combinations reported in the experimental section,
other than the official scores from WMT12 metrics task. For reproducibility, we refer below to the
individual metrics from \asiya\ with the exact names required by the toolkit to calculate them.

We departed from \asiya's ULC~\cite{AsiyaMTjournal:2010}, which was the
best performing metric at system and segment levels at the WMT08 and WMT09
metrics tasks. This is a  uniform linear combination of 12 individual metrics.
From the original ULC, defined in (Gim\'enez and M\`arquez, 2010a, pages 21--23),
we only replaced TER and Meteor individual metrics by newer versions taking into account
synonymy lookup and paraphrasing (`TERp-A' and `Meteor-pa' in \asiya's terminology).
We will call this combined metric \asiyaix\ in the experiments.

We also computed the scores of a few extra usual evaluation measures to complement
the metrics provided by system- and segment-level evaluation tables from WMT12 metrics task.
These are `BLEU' \cite{Papineni:Roukos:Ward:Zhu:2002}, `NIST' \cite{Doddington:2002:AEM}, 
`TER' \cite{Snover06astudy}, `ROUGE-W' \cite{Lin04}, and three Meteor variants \cite{Denkowski2011}, 
`Meteor-ex' (exact match), `Meteor-st' (+stemming) and `Meteor-sy' (+synonyms).
The uniform linear combination of the previous 7 individual metrics plus the 12 from \asiyaix\
was calculated with \asiya\ and reported as \asiyaall\ in the experimental section.

The individual metrics combined in \asiyaall\ can be naturally categorized according to the
type of linguistic information they use to compute the quality scores. We have grouped
them in the following four families and calculated again with \asiya\ the uniform linear
combination of the metrics in each group:\footnote{A detailed description of every individual
metric can be found at \cite{AsiyaMTjournal:2010}. For a more up-to-date description,
see the User Manual from \asiya's website.}\smallskip\\
%\begin{enumerate}
%\item \lex. Combination of five metrics based on lexical similarity:
%`BLEU', `NIST', `METEOR-ex', `ROUGE-W' and `TERp-A'.
%\item \syn. Combination of four metrics based on syntactic information
%coming from constituency and dependency parse trees:
%`CP-STM-4', `DP-HWCM\_c-4', `DP-HWCM\_r-4', and `DP-Or(*)'.
%\item \srl. Combination of three metric variants based on predicate argument structures
%(semantic role labeling): `SR-Mr(*)', `SR-Or(*)', and `SR-Or'.
%\item \dis. Combination of two metrics variants based on semantic parsing\footnote{In \asiya\
%the metrics from this family are said to be ``Discourse Representation'' metrics. However, the
%structures they consider are actually very different from the discourse structures exploited
%in this paper. See the discussion in Section~\ref{sec:related}.
%For clarity, we will refer to them as \emph{semantic parsing} metrics.}:
%`DR-Or(*)' and `DR-Orp(*)'.
%\end{enumerate}
%
\noindent (1) \lex. Combination of five metrics based on lexical similarity:
`BLEU', `NIST', `METEOR-ex', `ROUGE-W', and `TERp-A'.\smallskip\\
%
\noindent (2) \syn. Combination of 4 metrics based on syntactic information
 from constituency and dependency parse trees:
\hbox{`CP-STM-4'}, `DP-HWCM\_c-4', `DP-HWCM\_r-4', and `DP-Or(*)'.\smallskip\\
%
\noindent (3) \srl. Combination of three metric variants based on predicate argument structures
(semantic role labeling): `SR-Mr(*)', `SR-Or(*)', and `SR-Or'.\smallskip\\
%
\noindent (4) \dis. Combination of two metrics variants based on semantic parsing:\footnote{In \asiya \ 
the metrics from this family are said to be ``Discourse Representation'' metrics. However, the
structures they consider are actually very different from the discourse structures exploited
in this paper. See the discussion in Section~\ref{sec:related}.
For clarity, we will refer to them as \emph{semantic parsing} metrics.}
`DR-Or(*)' and `DR-Orp(*)'.

%\subsection{Data and Processing} \label{DataPreprocess}
\subsection{Human Judgements and Learning} \label{DataPreprocess}

The human-annotated data from the WMT campaigns encompasses series of rankings for the output of different MT systems for a particular source sentence. Annotators rank the output of five systems according to perceived translation quality.
%For each source segment, annotators were asked to rank five system submissions.
The organizers relied on random selection, and a large number of sample pairs to make comparisons across systems feasible \cite{WMT12}. As a result, for each source sentence, only relative rankings were available.

As in the WMT12 experimental setup, we use these rankings to calculate correlation with human judgments 
at the sentence level, i.e. Kendall's Tau; see \cite{WMT12} for detail.

For the experiments reported in Section~\ref{sec:results}.3, we also used the pairwise rankings to 
discriminatively learn the weights of the linear combinations of individual metrics.
%tune the weights of metric combinations, 
We followed the same approach used by PRO to tune the relative weights
of the components of a log-linear SMT model~\cite{Hopkins:2011}, also using Maximum Entropy as the 
base learning algorithm.\footnote{Unlike PRO,
\Ni \ we use \emph{human judgments}, not automatic scores, and
\Nii \ we train on \emph{all pairs}, not on a subsample.}
In order to use the WMT12 data for training a learning-to-rank model, we transformed the five-way relative rankings into ten pairwise comparisons. For instance, if a judge ranked the output of systems $A$, $B$, $C$, $D$, $E$ as $A>B>C>D>E$,
this would entail that $A>B$, $A>C$, $A>D$ and $A>E$, etc.%and so on.

%%% Lluís: son 10 no? (5*4)/2 el orden de cada par es solo uno

%%%% Lluís: part of the following is already covered in 5. Decide what to do with 4.3 and 4.4
%\subsection{Evaluation}
%When evaluating the performance of a MT metric, the standard procedure is to compare how well it correlates with human judgements. There are several ways this can be done. In this paper, we follow the WMT guidelines, and report Spearman's Rho for system level evaluation, and Kendall's Tau for segment level evaluation.
%
%\paragraph{System-level evaluation.}
%We measure the rank correlation of the metrics at a system level with the human judgements. To do so, we compute the {\it expected wins} (i.e. $wins/(wins+loses)$ ) for each system, based on how many times a system was ranked better than others ($wins$) and worse than others ($loses$), and use these to rank each of the systems accordingly to produce ranking $H$. Furthermore, we use the raw scores obtained from the metrics at a system level, and also use these to produce a raking $M$. Finally, we compute Spearman's Rho rank correlation over the rankings $H$ and $M$.
%
%\paragraph{Segment-level ranking.}
%
%\alert{This is going to move to 5??}
%\subsection{MaxEnt Combination}
%- - - Discourse and Current Metrics\\
%- - - Discourse as a Metric component (ASIYA)\\
%

